Topological Data Analysis of Spatial Patterning in Heterogeneous Cell Populations: Clustering and Sorting with Varying Cell-Cell Adhesion

Different cell types aggregate and sort into hierarchical architectures during the formation of animal tissues. The resulting spatial organization depends (in part) on the strength of adhesion of one cell type to itself relative to other cell types. However, automated and unsupervised classification of these multicellular spatial patterns remains challenging, particularly given their structural diversity and biological variability. Recent developments based on topological data analysis are intriguing to reveal similarities in tissue architecture, but these methods remain computationally expensive. In this article, we show that multicellular patterns organized from two interacting cell types can be efficiently represented through persistence images. Our optimized combination of dimensionality reduction via autoencoders, combined with hierarchical clustering, achieved high classification accuracy for simulations with constant cell numbers. We further demonstrate that persistence images can be normalized to improve classification for simulations with varying cell numbers due to proliferation. Finally, we systematically consider the importance of incorporating different topological features as well as information about each cell type to improve classification accuracy. We envision that topological machine learning based on persistence images will enable versatile and robust classification of complex tissue architectures that occur in development and disease.

==> sections/SI/0_ABM.tex <==
\subsection{Analytical Calculations for the ABM Model} 

In the absence of any random self-propulsion force, the equilibrium distance between particles, $r_{\text{eq}}$, is determined by the Morse potential parameters:

\begin{equation}
\label{eqn:ABM_Fexp}
    |\mathbf{F}_{ij}| = \gamma_{ij} \Bigg| \frac{1}{4l_R}\text{exp}\Big(-\frac{r_{ij}}{l_R}\Big)-\frac{1}{l_A}\text{exp}\Big(-\frac{r_{ij}}{l_A}\Big)\Bigg| = 0 \implies r_{\text{eq}}=\frac{l_Al_R}{l_A-l_R}\ln\Big(\frac{l_A}{4l_R}\Big) \approx 1.009
\end{equation}

The depth of the potential well is maximized at $r_{\text{eq}}$:

\begin{equation}
\label{eqn:ABM_Udepth}
    U(r_{\text{eq}}) = - \gamma_{ij} \Big( \frac{4l_R}{l_A}\Big)^\frac{l_R}{l_A-l_R} + \frac{\gamma_{ij}}{4} \Big( \frac{4l_R}{l_A}\Big)^\frac{l_A}{l_A-l_R} \approx -0.897 \gamma_{ij}
\end{equation}

\noindent The distance at which the force due to the Morse potential reaches local maximum lies outside the neighborhood distance $r_\text{max}$ (Eqn. \ref{eqn:ABM_dFdr}), therefore the maximum attraction and repulsion force occur at $r=r_\text{max}$ and $r=0$ respectively (Eqn. \ref{eqn:ABM_Fmax}):

\begin{equation}
\label{eqn:ABM_dFdr}
\frac{d|\mathbf{F}_{ij}|}{dr_{ij}} = 0 \implies r = \frac{l_Al_R}{l_A-l_R} \ln\Big(\frac{l_A^2}{4l_R^2}\Big) \approx 2.737 > r_{\text{max}}
\end{equation}

\begin{equation}
\label{eqn:ABM_Fmax}
    |\mathbf{F}_{ij}|_{\text{max}} = \begin{cases}
      \displaystyle
      \frac{l_A-4l_R}{4l_Al_R}\max(\gamma_{ij}) \approx 0.4286 \max(\gamma_{ij}), & \text{at}\ r_{ij}=0 \\
      \Big|\frac{1}{4l_R}\text{exp}\Big(-\frac{r_\text{max}}{l_R}\Big)-\frac{1}{l_A}\text{exp}\Big(-\frac{r_\text{max}}{l_A}\Big)\Big|\max(\gamma_{ij}) \approx 0.0393 \max(\gamma_{ij}), & \text{at}\ r_{ij}=r_\text{max}
      \end{cases}
\end{equation}

The ratio between the maximum attractive force and the polarization force varies between $0.078$ and $1.964$ for adhesion energy values $\gamma_{ij} \in [0.01, 0.25]$ and fixed polarization force magnitude, $|\mathbf{P}| = 0.005$. In a binary system, the polarization force dominates over the attractive adhesion force when $\gamma_{ij} < 0.127$. \textbf{TODO: account for random polarization}

\begin{equation}
\label{eqn:ABM_force_ratio}
0.078 < \frac{|\mathbf{F}_{ij}^{\text{attr}}|}{|\mathbf{P}_i|} = \frac{0.0393\gamma_{ij}}{0.005} < 1.964
\end{equation}


==> sections/abstract.tex <==
Animal tissues are comprised of multiple cell types that self-sort and cluster into rich topological patterns based on differences in cell-cell adhesion. For instance, zebrafish exhibit a variety of striped skin patterns, while fruit flies can exhibit distinct tissue compartments as well as hierarchical hexagonal patterning in the retina. Automated classification of these patterns can be challenging, since cells may exhibit non-uniform spacing, as well as variability in local number and density. Topological data analysis is a promising approach that uses persistent homology to visualize the spatial connectivity between discrete cell positions, and to determine the topological similarity of different patterns. Here, we demonstrate unsupervised classification of hierarchical tissue patterns comprised of two different cell types by considering the topological configurations of each cell type and of all cells combined. We first validate this approach by systematically varying interactions between two cell types at fixed population size, and then consider the effect of including proliferation that is spatially limited by contact inhibition. We further consider the classification of zebrafish stripe patterns associated with various mutations, and evaluate the stability of this analysis when these patterns are synthetically distorted. Overall, this work shows that topological analyses are highly effective for machine learning of multiscale spatial patterns that incorporate several different components, which may yield new insights into the emergence of larger scale tissue architectures in development and disease.

==> sections/discussion.tex <==
\section{\label{sec:discuss}Discussion and Conclusion}

We demonstrate a generalizable topological framework to classify spot and stripe patterns comprised of two interacting cell types. Our approach utilizes persistence images as a finite vector representation of persistence diagrams, which is a standardized format for machine learning \cite{Adams2017}. Briefly, discrete points on the persistence diagram with some coordinates (birth $b$, persistence $d-b$) are replaced by Gaussian distributions centered on each point. This use of persistence images permits direct comparison of multicellular patterns with varying population size without the arbitrary normalization needed for connected components in persistence diagrams. Next, the weighted sum of these Gaussians represents a surface, which is discretized as a grid to generate a vector. In this work, we choose a weighting by $(d-b)^2$, which emphasizes more persistent features. We show that these persistence images retain information about structural features that manifest at larger length scales, due in part to this weighting. Thus, persistence images can outperform conventional order parameters (e.g. radial distribution function) where structural information at large distances is washed out by noise after ensemble-averaging of cell (particle) positions with high variability. Finally, persistence images can be manipulated and analyzed with much greater computational efficiency. Wasserstein distance computation requires an optimal transport plan between persistence diagrams, which is more expensive to compute in comparison to Euclidean distances between Gaussian-weighted persistence images. 

%\textbf{Jay add a few more sentences here}
 
To validate this approach, a discrete agent model was implemented using two cell types with tunable homotypic and heterotypic adhesion. Remarkably, this minimal model recapitulated a variety of multicellular patterns observed in animal tissues, including self-sorted individuals or aggregates, encapsulated clusters, stripes, hexagonal configurations, and labyrinth-like architectures (\textbf{Fig.~\ref{fig:phasediagramnoprolif}}). \textbf{Comment on most effective TDA approach}. It should be noted that these simulated discrete agents were of identical size and shape, and the relative uniformity in cell-cell spacing can be captured by conventional order parameters (e.g. radial distribution function). However, living cells in actual animal tissues exhibit a more heterogeneous size distribution, which will increase the variability in cell-cell spacing and likely confound radial distribution functions by averaging out positional information. Moreover, epithelial tissues consist of deformable cells that are tightly packed in polygonal geometries, which are often simulated using vertex models \cite{Alt:2017cp}. Nevertheless, we anticipate that these disordered cell configurations exhibit persistent topological features that can still be effectively classified by TDA, which represents an exciting direction for future work. 

\textbf{Placeholder -add discussion on zebrafish stripes} - note lack of finite size effects, and also that whatever is not a melanophore is a xanthophore

Although this initial proof of concept addressed two interacting cell types in a planar geometry, it should be noted that these topological methods are generalizable to multiple cell types on a non-planar geometry. For instance, the establishment of a multilayered body plan in an embryo (gastrulation) involves coordinated migration of cells into new locations with new neighbors, which drive cell fate decisions \cite{barresi_gilbert_2020}. Such morphogenetic processes such as invagination, involution, ingression, delamination, or epiboly, will arguably result in dramatically different topologies with distinct persistent features. Given the wealth of spatial and temporal information enabled by modern live cell imaging techniques \cite{Keller:2013ha}, TDA has great potential to classify and interpret cell shape changes, division, migration, and growth within the embryo. Finally, these spatial descriptors could be further integrated with single cell gene expression profiling, which have also utilized topological (manifold-learning) analyses \cite{Wagner:2020bp}. 

==> sections/intro.tex <==
\section{\label{sec:intro}Introduction}

Animal tissues are spatially organized into complex topologies by heterotypic interactions between different cell types \cite{Lecuit:2007cw}. For instance, mixtures of animal cells in a flat monolayer can self-sort into their respective types, as well as aggregate into multicellular clusters \cite{Graner:1992kx,Rieu:1998bf,Belmonte:2008dv,Hogan:2009bc,Beatrici:2011fz,Mehes:2012fy,Kabla:2012gm,Strandkvist:2014ie,Nielsen:2015jl,GamboaCastro:2016da,Leggett:2019hva,Li:2019bt,Krajnc:2020dd,Sahu:2020cc,Dey:2021ke}. Steinberg sought to explain these behaviors using a physical analogy with surface tension, where cells exhibit ``differential adhesion'' with one another \cite{Steinberg:2007ih}. For instance, two different cell types that each exhibit strong homotypic adhesion (to self) but weak heterotypic adhesion (to the other) would eventually segregate into separate clusters, each consisting of a single cell type  \cite{Steinberg:1963kq}. Instead, two cell types, each with strong heterotypic adhesion (to the other) would randomly intermix within a single cluster. Between these limiting cases, intermediate homotypic and heterotypic adhesion would result in a core-shell organization, where a first cell type would aggregate at the interior, and the second cell type would organize as a spread layer around the periphery. More recent work using \emph{Drosophila melanogaster} has addressed the importance of cellular contractility \cite{kasza2011dynamics} and proliferation \cite{Gibson:2006gi} in tissue patterning, resulting in distinctive topologies including developmental compartment boundaries \cite{Major:2006ir}, hierarchical hexagonal patterning in the retina \cite{Hayashi:2004it}, as well as multicellular rosettes during germband extension \cite{Blankenship:2006jg}. Zebrafish (\emph{Danio rerio}) has also been used as a model system for skin tissue patterning, exhibiting a variety of striped phases on based on the self-organization of three cell types: black melanophores, yellow / orange xanthophores, and iridescent silver/blue iridophores \cite{Volkening:2020jd}. More complicated finger-like or labyrinth-like tissue patterning has been attributed to reaction-diffusion (Turing) mechanisms \cite{Kondo:2010bx}, and have also been elucidated using on-lattice \cite{Bullara2015} or off-lattice discrete agent models \cite{Volkening2015,Volkening2018}. Given this rich diversity of tissue topologies generated experimentally and in silico, an emerging challenge is to achieve an automated and unbiased classification of distinct spatial patterns \cite{bishop_2016}.  An intriguing possibility is to implement an interpretable and computationally-efficient machine learning framework that can be generalized to classify spatial patterns comprised of multiple interacting cell types.

Topological data analysis (TDA) is a promising approach for machine learning of high-dimensional architectures that extracts the ``shape'' of a dataset based on spatial connectivity \cite{carlsson2009topology}. TDA considers how data points may be connected pairwise (dimension 0 homology) or linked into closed loops around an empty region (dimension 1 homology), then examines the stability of these connected structures at varying spatial scales (i.e. persistent homology) \cite{herbertedelsbrunner2009}. Topological features can then be represented using a characteristic persistence ``barcode'' or ``diagram,'' and their relative ``similarity'' can be determined based on the ``cost'' of rearranging one diagram to resemble the other \cite{Amezquita:2020bi}. Alternatively, persistence images represent topological features based on the weighted sum of Gaussian features, which yields a standardized finite vector representation that is amenable for machine learning \cite{Adams2017}. Such topological approaches have recently been used to visualize the spatial organization of a single motile species \cite{Topaz:2015gd, Ulmer:2019hx, atienza2019persistent, Bhaskar:2019hj, McGuirl201917763, skinner2021topological} and particulate systems \cite{kramar_quantifying_2014}. These past investigations mostly utilized connected components (dimension 0 homology) to analyze populations of fixed size that were near confluency. One drawback of this approach is that the number of connected components scales with the size of the population, which will bias the classification when different populations have different sizes. Our recent work has shown that classification based on closed loops (dimension 1 homology) is a highly robust approach to classify spatial patterns with varying population size, particularly in the presence of empty regions \cite{bhaskar2020topological}. Nevertheless, the effectiveness of TDA for classifying spatial patterns comprised of multiple species has not been previously addressed.

In this article, we show that TDA enables unsupervised classification of spatial patterns that emerge from two interacting cell types by considering dimension 0 and 1 homology for each cell type and with both cell types combined. We systematically tune homotypic and heterotypic interactions between cell types to generate distinct architectures ranging from dispersed individuals to intermixed clusters to partially or wholly sorted clusters, as well as more complex striped phases, hierarchical hexagonal patterns, and rosettes. We evaluate the classification accuracy of TDA for a population of constant size, as well as when cells can undergo spatially limited proliferation. As a case study, we further apply TDA to analyze zebrafish stripe patterns associated with various mutations. This work establishes the importance of accounting for topological structure associated with both species, as well as special cases where TDA of only one species is sufficient for effective classification. We envision this computational approach will enable new quantitative insights into the emergence of complex tissue topologies via spatiotemporal interactions between multiple cell types \cite{Goodwin:2017fb}.

==> sections/methods.tex <==
\section{\label{sec:methods}Methods}

\input{sections/methods/0_ABM}

\input{sections/methods/1_TDA}

\input{sections/methods/3_OP}

==> sections/methods/0_ABM.tex <==
\subsection{\label{sec:abm}Agent-Based Model}

Cells were first represented as rigid-body agents that undergo non-inertial motion (Eqn. \ref{eqn:ABM_FE}) due to random self-propulsion force, $\mathbf{P}$, and cell-cell interactions governed by the attraction-repulsion force, $\mathbf{F}$. Cell positions are initialized in a $[-20,20]\times[-20,20]$ simulation box with periodic boundaries on all sides. The equation of motion is given by:

\begin{equation}
\label{eqn:ABM_FE}
    \mathbf{x}_i^{t+\Delta t} = \mathbf{x}_i^t + \frac{\Delta t}{\eta}\Big( \mathbf{P}_i^t + \sum_{j \ne i}^{N(t)} \mathbf{F}_{ij}^t \Big)
\end{equation}

where $\mathbf{x}_i^t$ denotes the position of the $i$th cell at time $t$, $\Delta t$ denotes the timestep, and $\eta$ denotes a friction coefficient.

\noindent Two cells $i$ and $j$ in close proximity (within neighborhood distance $r_{\text{max}} = 1.5$) can attract or repel each other in accordance with an the attraction-repulsion force, $\mathbf{F}$ that is the gradient of the Morse potential, $U$ (Eqn. \ref{eqn:ABM_Adh}). This potential function (Eqn. \ref{eqn:ABM_U}) is characterized by length scales $l_A=14.0$ and $l_R=0.5$ for long-range attraction and short-range repulsion respectively. The second short-range repulsion term was further scaled to be 1/4 of the first long-range attraction term. 

\begin{equation}
\label{eqn:ABM_Adh}
    \mathbf{F}_{ij} = -\nabla U(||\mathbf{x}_j-\mathbf{x}_i||) \frac{\mathbf{x}_j - \mathbf{x}_i}{||\mathbf{x}_j - \mathbf{x}_i||} \mathbf{1}_{||\mathbf{x}_j - \mathbf{x}_i|| \le r_{\text{max}}}
\end{equation}

\begin{equation}
\label{eqn:ABM_U}
    U(r_{ij}) = -\gamma_{ij}\Bigg(\text{exp}\Big(\frac{-r_{ij}}{l_A}\Big)-\frac{1}{4}\text{exp}\Big({-\frac{r_{ij}}{l_R}}\Big)\Bigg)
\end{equation}

\noindent The magnitude of the attraction-repulsion force is determined by the adhesion parameter $\gamma_{ij} = \gamma(T(i),T(j))$, which depends on cell types $T(i)$ and $T(j)$ for cells $i$ and $j$ respectively. Here we consider two cell types, shown in blue and orange, with cell types denoted by $\tau_B$ and $\tau_O$ respectively.\\

\noindent Cell positions are initialized at $t=0$ from a uniform distribution with rejection sampling to ensure a minimum separation of $1.0$ between all cells. The magnitude of the polarization force, $|\mathbf{P}|$, is fixed at $0.005$ and the adhesion parameter, $\gamma$, is varied between $0.01$ and $0.25$.\\

The friction coefficient $\eta=1.0$, and time-step $\Delta t = 0.02$, are constant throughout the simulation. Each simulation ran for $5,000,000$ time-steps. Repolarization takes place every $2,500$ time-steps, with an initial offset to prevent synchronization. In cases where cell division is turned on, the cell cycle duration is set to $80,000$ time-steps.

==> sections/methods/1_TDA.tex <==
\subsection{\label{sec:tda}TDA \& Persistence Diagrams}

\subsection{\label{sec:persimg}Persistence Image Computation}

Given a persistence diagram $\mathcal{D}$ corresponding to homology group $H_n (n > 0)$, its persistence image is obtained by superimposing weighted Gaussian kernels, $g$, at each point $(b,d) \in \mathcal{D}$:

\begin{equation}
\label{eqn:PI_Hn}
\text{PI}(x,y; H_n) = \sum_{(b,d)\in\mathcal{D}} (d-b) \cdot g_{(b,d-b),\Sigma}(x,y) \quad x \in [0, \epsilon_{\text{max}}] \quad y \in \Big[0, \frac{\epsilon_{\text{max}}}{2}\Big]
\end{equation}

where the Gaussian kernel is parameterized by mean $\mathbf{\mu}$ and covariance matrix $\Sigma$:

\begin{equation}
\label{eqn:Gauss_2D}
g_{\mathbf{\mu},\Sigma}(\mathbf{x}) = \frac{\text{exp}(-\frac{1}{2}(\mathbf{x}-\mathbf{\mu})^T\Sigma^{-1}(\mathbf{x}-\mathbf{\mu}))}{2\pi |\Sigma|^{1/2}}
\end{equation}

In practice an isotropic kernel with $\Sigma = \sigma^2 \cdot I_2$ is used. The weights $d - b$ ensure that points further from the diagonal, corresponding to more significant topological features have greater contribution. The persistence diagram for the $0^{\text{th}}$ homology group ($H_0$), contains intervals that share birth time, $b=0$. In this case, the persistence image is 1-D:

\begin{equation}
\label{eqn:PI_H0}
\text{PI}(x; H_0) = \sum_{(b,d)\in\mathcal{D}} (d-b) \cdot g_{d-b,\sigma^2}(x) \quad x \in [0, \epsilon_{\text{max}}]
\end{equation}

where the 1-D Gaussian kernel is specified as follows:

\begin{equation}
\label{eqn:Gauss_1D}
g_{\mu,\sigma^2}(x) = \frac{1}{\sqrt{2\pi}\sigma}\text{exp}\Big(-\frac{1}{2}\frac{(x-\mu)^2}{\sigma^2}\Big)
\end{equation}

\subsection{\label{sec:perscurve}Persistence Curve Computation}

Given a persistence diagram $\mathcal{D}$, corresponding to the $n^\text{th}$ homology group, the Gaussian persistence curve is defined as \cite{chung_smooth_2020}:

\begin{equation}
\label{eqn:PC_Hn}
\text{PC}(t; H_n) = \int_t^{\infty} \int_{-\infty}^t \sum_{(b,d)\in\mathcal{D}} (d-b) \cdot g_{(b,d),\Sigma}(x,y) dx dy \quad \text{for} \quad t \in [0, \epsilon_{\text{max}}]
\end{equation}

with 2-D Gaussian kernel $g$ as defined in Eqn. \ref{eqn:Gauss_2D}. Assuming, $\Sigma = \sigma^2 \cdot I_2$, the Gaussian is separable

\begin{equation}
\label{eqn:PC_cdf}
\text{PC}(t; H_n) = \sum_{(b,d)\in\mathcal{D}} (d-b) \cdot G_{b,\sigma^2}(t)(1-G_{d,\sigma^2}(t)) \quad \text{for} \quad t \in [0, \epsilon_{\text{max}}]
\end{equation}

where $G$ is the c.d.f of the 1-D Gaussian kernel $g$ (Eqn. \ref{eqn:Gauss_1D}). We normalize the persistence curve by the number of intervals in the persistence diagram:

\begin{equation}
\text{NPC}(t; H_n) = \begin{cases}
      \frac{1}{|\mathcal{D}|} \text{PC}(t; H_n), & \text{if}\ |\mathcal{D}|>0 \\
      0, & \text{otherwise}
    \end{cases}
\end{equation}

==> sections/methods/3_OP.tex <==
\subsection{\label{sec:orderparam}Order Parameters}

Particle position $\mathbf{x}_i=(x_i, y_i)$ is expressed in polar coordinates $(r_i,\theta_i)$. Recall from Section \ref{sec:abm} that total number of cells is $N = N_B + N_O$. For each particle $i$, it's type is denoted by $\tau(i)$. Blue cells have type $\tau_B$ and orange cells have type $\tau_O$. Angular distribution is characterized by $3$ order parameters:

\begin{equation}
\begin{aligned}
    \Theta(\theta) &= \frac{1}{N^2}\sum_{i=1}^N\sum_{j=1}^N \mathbf{1}_{\theta-d\theta \le \theta_j - \theta_i \le \theta + d\theta}\\
    \Theta_B(\theta) &= \frac{1}{N^2}\sum_{i=1}^N\sum_{j=1}^N \mathbf{1}_{\theta-d\theta \le \theta_j - \theta_i \le \theta + d\theta} \cdot \mathbf{1}_{\tau(j)=\tau_B}\\
    \Theta_O(\theta) &= \frac{1}{N^2}\sum_{i=1}^N\sum_{j=1}^N \mathbf{1}_{\theta-d\theta \le \theta_j - \theta_i \le \theta + d\theta} \cdot \mathbf{1}_{\tau(j)=\tau_O}
\end{aligned}
\end{equation}

Note that:

\begin{equation*}
\begin{aligned}
    \sum_\theta \Theta(\theta) &= 1\\
    \sum_\theta \Theta_B(\theta) &= \frac{N_B}{N}\\
    \sum_\theta \Theta_O(\theta) &= \frac{N_O}{N}
\end{aligned}
\end{equation*}

\noindent Radial distribution of particle density is characterized by counting average number of neighbors within distance $r$ of each cell:

\begin{equation}
\begin{aligned}
    R(r) &= \frac{1}{N^2} \sum_{i=1}^N \sum_{j=1}^N \mathbf{1}_{||\mathbf{x}_j-\mathbf{x}_i||\le r}\\
    R_B(r) &= \frac{1}{N^2} \sum_{i=1}^N \sum_{j=1}^N \mathbf{1}_{||\mathbf{x}_j-\mathbf{x}_i||\le r} \cdot \mathbf{1}_{\tau(j)=\tau_B}\\
    R_O(r) &= \frac{1}{N^2} \sum_{i=1}^N \sum_{j=1}^N \mathbf{1}_{||\mathbf{x}_j-\mathbf{x}_i||\le r} \cdot \mathbf{1}_{\tau(j)=\tau_O}
\end{aligned}
\end{equation}

Observe:

\begin{equation*}
\begin{aligned}
    \displaystyle \lim_{r \rightarrow \infty} R(r) &= 1\\
    \displaystyle \lim_{r \rightarrow \infty} R_B(r) &= \frac{N_B}{N}\\
    \displaystyle \lim_{r \rightarrow \infty} R_O(r) &= \frac{N_O}{N}
\end{aligned}
\end{equation*}

\noindent Degree of cell sorting or mixing is characterized by counting the average number of heterotypic neighbors within radius $r$ (similar to \cite{belmonte_self-propelled_2008}):

\begin{equation}
\begin{aligned}
    \widetilde{R}(r) &= \frac{1}{N^2} \sum_{i=1}^N \sum_{j=1}^N \mathbf{1}_{||\mathbf{x}_j-\mathbf{x}_i||\le r} \cdot \mathbf{1}_{\tau(i)\ne\tau(j)}\\
    \widetilde{R}_B(r) &= \frac{1}{N \cdot N_B} \sum_{i=1}^N \sum_{j=1}^N \mathbf{1}_{||\mathbf{x}_j-\mathbf{x}_i||\le r} \cdot \mathbf{1}_{\tau(i)=\tau_B\land\tau(j)=\tau_O}\\
    \widetilde{R}_O(r) &= \frac{1}{N \cdot N_O} \sum_{i=1}^N \sum_{j=1}^N \mathbf{1}_{||\mathbf{x}_j-\mathbf{x}_i||\le r} \cdot \mathbf{1}_{\tau(i)=\tau_O\land\tau(j)=\tau_B}
\end{aligned}
\end{equation}

Observe:

\begin{equation*}
\begin{aligned}
    \displaystyle \lim_{r \rightarrow \infty} \widetilde{R}(r) &= \frac{2 \cdot N_B \cdot N_O}{N^2} \Big[ = \frac{1}{N} (\text{Harmonic Mean}) \Big]\\
    \displaystyle \lim_{r \rightarrow \infty} \widetilde{R}_B(r) &= \frac{N_O}{N}\\
    \displaystyle \lim_{r \rightarrow \infty} \widetilde{R}_O(r) &= \frac{N_B}{N}
\end{aligned}
\end{equation*}

==> sections/results.tex <==
\section{\label{sec:results}Results}

\input{sections/results/0_TDA}

\input{sections/results/1_ABM}

==> sections/results/0_TDA.tex <==
\subsection{Classification Using Persistence Images}

Given a point cloud representation of cell positions, we extract topological features such as connected components (dimension 0 homology) and loops (dimension 1 homology) using persistent homology. Intuitively, we expand an $\epsilon$ radius ball, $B_p(\epsilon)$ around each point $p$, connecting pairs of points with an edge, three points with a filled-in triangle, four points with a tetrahedron, and so on, as the balls intersect in a pairwise manner. This construction is formalized in algebraic topology as the Vietoris-Rips filtration. For example, consider dimension 0 homology when $\epsilon = 0$. We have $N$ connected components and no loops, supposing that $N$ represents the total number of points in the point cloud. We would mark these features as being born at radius 0. Suppose that these epsilon balls later first intersect at a radius $\epsilon = d$. Then we say that the original features (except for one) of the individual points have died at radius $d$. Observe that all connected components are born at radius $\epsilon = 0$, and as $\epsilon \to \infty$, all connected components will die except for one. We record the birth and death radii for all such topological features, including loops for dimension 1, which have variable birth and death unlike connected components. By this process, we have generated a set of $[birth,death)$ intervals for the topological features, which we call the persistence of the feature, and a larger $death - birth$ corresponds to a more persisting feature, and thus a more significant one. These birth and death pairs can be represented using a barcode diagram, or a persistence diagram where we plot $(birth,death)$.

In order to encode this information into vectors such that it is conducive to machine learning, we use persistence images\cite{Adams2017}. Generally, in order to compute a persistence image, we take the points from the persistence diagram and place Gaussians centered around each point, additionally weighting the Gaussians so that more significant points are more represented. Then we take the sum over these Gaussians.

For dimension 0 homology, we consider only the connected component features and place Gaussians at each point weighted by $(death - birth)$ so we get a 1-dimensional intensity function of the birth radius. Mathematically,

\begin{align*}
    PI(x) = \sum\limits_{(birth,death) \in \mathcal{D}} (death - birth) g_{(birth),\sigma}(x)
\end{align*} 

where $\mathcal{D}$ is the persistence diagram and $g_{(birth),\sigma}$ is a Gaussian with mean $birth$ and variance $\sigma^{2}$\\

For the dimension 1 homology, we consider only the loops and we change coordinates from $(birth, death)$ to $(birth, death - birth)$ and place Gaussians around these new points, weighted by the distance to the diagonal where $birth = death$. In other words, we weight each Guassian by $\sqrt{(\frac{birth - death}{2})^{2} + (\frac{death - birth}{2})^{2}}$. The result is a 2-dimensional intensity function, with higher intensity for more persisting features. Mathematically,

\begin{align*}
    PI(x,y) = \sum\limits_{(birth,death) \in \mathcal{D}} (death - birth) g_{(birth,death - birth),\Sigma}(x,y)
\end{align*} 

where $g_{(birth,death - birth),\Sigma}$ is a 2-dimensional Gaussian with mean $(birth,death - birth)$ and covariance matrix $\Sigma$. This can be generalized to higher dimension homologies.

Persistence curves are an alternative method of summarizing the persistence diagram. Starting with the persistence diagram, we define a function on the diagonal of the persistence diagram. Let $t$ be a point on the diagonal, such that $t= (b,d)$ for $b = d$. Now we look at the rectangular region where $birth \leq b$ and $death \geq d$. We then apply some function $\psi$ over the points within this region and that output will be $P(t)$. More formally, we define the mapping $\textsc{PC}: \mathcal{D} \times \Psi \times \mathcal{T}$ to be 

\begin{align*}
    \textsc{PC}(D,\psi,T)(t) = T(\psi(D;b,d,t)|(b,d)\in D_{t}), t\in \mathcal{R} 
\end{align*} 

where $D$ is the persistence diagram, $\psi$ is the function applied to points in the region, and $T$ is a summary statistic that maps from a set of points to a real number \cite{chung_smooth_2020}. 

The functions $\psi$ and $T$ in combination have many varieties. For example, we can simply count the number of points in the region, normalized by the total number of points. This is called the Betti curve. Another option is to sum the total $death - birth$ in the region, which is also called the total life in the region, which results in a Life curve. Finally, another possibility is the Gaussian Persistence Curve, which places Gaussians on each of the points within the region and integrates over the region. There are many other possible $\psi$ functions that could be applied, each with different ways of encoding information. Some benefits of using persistence curves are efficiency: they are easy to implement and fast to compute, as well as flexible due to the choice of $T$ and $\psi$, and there are theoretical results for convergence and boundedness.

%% EXAMPLE PLACEHOLDER TEXT FROM NARDINI - MUST REWRITE!! %%

%PH is an algorithm that takes in data via a filtration and outputs a quantification of topological features such as connected components (dimension 0) and loops (dimension 1) across the filtration. The simplicial complexes are indexed by the scale parameter of the filtration. In our case, the scale parameter corresponds to the spatial location in the sweeping plane filtration or steps of flooding in the flooding filtration. Note that we compute these filtrations on simulated blood vessel network images at the final time step of a model simulation. The inclusion of a simplicial complex $Ki  \subseteq Kj$ for $i \le j$ gives a relationship between the corresponding homology groups $Hp(Ki)$ and $Hp(Kj)$ for $p = 0, 1$. This relationship enables us to track topological features such as loops along the simplicial complexes in the filtration. Intuitively, a topological feature is born in filtration step b when it is first computed as part of the homology group $Hp(Kb)$ and dies in filtration step d when that feature no longer exists in $Hp(Kd)$, i.e., when a connected component merges with another component or when a loop is covered by 2-simplices. The output from PH is a multiset of intervals $[b, d)$ which quantifies the persistence of topological features. Each topological feature is said to persist for the scale $d − b$ in the filtration. Our topological descriptors are the connected components (i.e., 0-dimensional) and loops (i.e., 1-dimensional features) obtained by computing persistent homology of the sweeping plane and flooding filtrations. We use the superscript notation $Kv$ to denote the filtered simplicial complex K in direction $v = {LTR, RTL, TTB, BTT, flood}$.

%Persistence images. A persistence image [52] uses as input the birth-death pairs given by PH and converts the set of (birth $b$, persistence $(d − b)$) coordinates into a vector, a format which is suitable for machine learning and other classification tasks. Following the standard definition of a persistence image, the coordinates $(b, d − b)$ are blurred by a Gaussian, with standard deviation $\sigma$, that is centered about each birth-persistence point, which accounts for uncertainty. We take a weighted sum of the Gaussians and place a grid on this surface to create a vector. We compute two alternative weighting strategies: all ones (in which case all features are equally weighted) and a persistence weight of $(d − b)$ (in which more persistent features are given larger weights). Let $PIOi(Kv)$ and $PIRi(Kv)$ denote the corresponding persistence images computed from $Kv$ with equal and ramped weighting, respectively, for dimension $i = {0, 1}$.
%The topological descriptor vectors that we compute for each model simulation are $\beta_i(Kv)$, $PIOi(Kv)$, and $PIRi(Kv)$, where $i = {0, 1}$ and $v = {LTR, RTL, TTB, BTT, flood}$. In total each simulation has $3 \times 2 \times 5 = 30$ topological descriptor vectors.

%We use an unsupervised algorithm, k-means clustering, to group the quantitative descriptor vectors of the synthetic data generated from simulations of the Anderson-Chaplain model. To cluster n samples  into k clusters, the k-means algorithm finds k points in , clusters each sample according to which of the k means it is closest to, and then minimizes the within-cluster residual sum of squares distance [58]. We cluster the standard descriptor vectors and the topological descriptor vectors (see steps 2A and 2B of the methods pipeline in Fig 2), respectively, to investigate whether descriptor vectors lead to biologically interpretable clusters.

%We test the robustness of each clustering assignment by randomly splitting the descriptor vectors into training and testing sets, and use the testing set to evaluate out-of-sample (OOS) accuracy. Specifically, 7 of the 10 descriptor vectors from each of the 121 (ρ, χ) parameter combinations are randomly chosen with uniform sampling and placed into a training set (847 simulations); the remaining 3 descriptor vectors from each (ρ, χ) combination are placed into a testing set (363 simulations). After performing unsupervised clustering with a k-means model on the training set, each (ρ, χ) combination is labeled by the majority of cluster assignments among its 7 training simulation descriptor vectors. To evaluate each clustering model’s OOS accuracy, the 3 test data samples for each (ρ, χ) parameter combination are given a “ground-truth” label equal to the cluster assignment for the 7 training simulations for that same (ρ, χ) parameter combination. A “predicted” label is calculated for each descriptor vector from the test data using the trained k-means model, and OOS accuracy is defined as the proportion of test simulations for which the “predicted” label matches the “ground-truth” label. For example, if the seven training simulations from the parameter combination (ρ, χ) = (0.2, 0.2) are placed into clusters {1, 1, 2, 2, 1, 1, 1}, then the three testing simulations from (ρ, χ) = (0.2, 0.2) will be labeled as being in cluster 1. If the test simulations are predicted to be from clusters {1, 2, 1}, then we compute an OOS accuracy of 66.67\%. We use all 363 testing simulations when computing OOS accuracy and use the KMeans command from scikit-learn (version 0.22.1), which uses Lloyd’s algorithm for Euclidean space, for training and prediction.

%% EXAMPLE PLACEHOLDER TEXT FROM NARDINI - MUST REWRITE!! %%

\begin{figure}
    \centering
    \includegraphics[width=10cm]{figures/persistence_image.png}
    \caption{\footnotesize \textbf{Computation of persistence image.} (A) Particle positions represented as a point cloud. (B) Persistence diagram computed using Vietoris-Rips complex. (C) Persistence image computed by summation of weighted 1-D Gaussians at each point (square) in the dimension 0 persistence diagram. (D) 2-D Gaussians with fixed bandwidth placed at each point (triangle) in the dimension 1 persistence diagram. (E) Switching the y coordinate to interval length (death - birth) and re-weighting by distance from the diagonal.}
    \label{fig:SI_persimg}
\end{figure}

==> sections/results/1_ABM.tex <==
\subsection{Sorting and Clustering of Two Non-Proliferating Cell Types with Varying Adhesion}

Differential adhesion simulations were performed using a self-propelled particle model with randomly initialized particle positions and periodic boundaries. Two cell types, labelled in blue ($\tau_B$) and orange ($\tau_O$), were simulated at constant population size ($N = 200$ total, $60\%$ blue and $40\%$ orange) by systematically varying parameters governing blue-blue adhesion ($\gamma_{BB}$), orange-orange adhesion ($\gamma_{OO}$), and blue-orange adhesion  ($\gamma_{OB}$), respectively. A random self-propulsion force of constant magnitude, $|\mathbf{P}|=0.005$ was applied to each particle throughout the simulation. The total simulation time was chosen to exceed the time taken to reach stable steady-state configurations for each set of parameter values. 

In the limit of zero orange-blue adhesion ($\gamma_{OB} = 0$) with weak blue-blue adhesion ($\gamma_{BB} < 0.03$) and weak orange-orange adhesion ($\gamma_{OO} < 0.03$), both orange and blue cells remained individually dispersed  (\textbf{Fig.~\ref{fig:phasediagramnoprolif}a,i}). At stronger blue-blue adhesion ($0.03 < \gamma_{BB}$) and weak orange-orange adhesion ($\gamma_{OO} < 0.03$), blue cells aggregated into clusters while orange cells remained individually dispersed (\textbf{Fig.~\ref{fig:phasediagramnoprolif}a,ii}). Conversely, at stronger orange-orange adhesion ($0.03 < \gamma_{OO}$) and weak blue-blue adhesion  ($\gamma_{BB} < 0.03$), orange cells aggregated into clusters while blue cells remained individually dispersed (\textbf{Fig.~\ref{fig:phasediagramnoprolif}a,iii}). Finally, at stronger blue-blue adhesion ($0.03 < \gamma_{BB}$) and stronger orange-orange adhesion ($0.03 < \gamma_{OO}$), blue cells aggregated into clusters and orange cells aggregated separately into clusters (\textbf{Fig.~\ref{fig:phasediagramnoprolif}a,iv}).

\begin{figure}
    \centering
    \includegraphics[width=12cm]{figures/noproliferationphasediagram.png}
    \caption{\textbf{Comparison of cluster and stripe patterning for two cell types (orange, blue) at constant population size with systematically varying blue-blue adhesion ($\gamma_{BB}$), orange-orange adhesion ($\gamma_{OO}$), and blue-orange adhesion  ($\gamma_{OB}$), respectively}. Representative slices with $\gamma_{BB}$ vs $\gamma_{OO}$ for $\gamma_{OB} = 0.0$ (a), $\gamma_{OB} = 0.05$ (b), $\gamma_{OB} = 0.13$ (c), $\gamma_{OB} = 0.25$ (d).}
    \label{fig:phasediagramnoprolif}
\end{figure}

At slightly increased orange-blue adhesion ($\gamma_{OB} = 0.05$), with comparable blue-blue ($\gamma_{BB} = 0.05$) or orange-orange adhesion ($\gamma_{OO} = 0.05$), sorting into separate blue and orange clusters was again observed (\textbf{Fig.~\ref{fig:phasediagramnoprolif}b,iv}). When blue-blue or orange-orange adhesions were stronger than orange-blue ($\gamma_{OB} \le \gamma_{OO}, \gamma_{OB} \le \gamma_{BB}$), a new type of cluster was observed with intermixed orange and blue cells (\textbf{Fig.~\ref{fig:phasediagramnoprolif}b,v}). Moreover, for weak blue-blue adhesion ($\gamma_{BB} < 0.03$) and weak orange-orange adhesion ($\gamma_{OO} < 0.05$), blue and orange cells organized into clusters with alternating stripes that were roughly 1-2 cells thick (\textbf{Fig.~\ref{fig:phasediagramnoprolif}b,vi}). These striped phases are analogous to those observed during skin patterning in zebrafish \cite{Volkening:2020jd}. At stronger blue-blue adhesion ($0.03 < \gamma_{BB}$) and weak orange-orange adhesion ($\gamma_{OO} < 0.03$), clusters consisted of orange cells dispersed in a hexagonal configuration, surrounded by blue cells.  (\textbf{Fig.~\ref{fig:phasediagramnoprolif}b,vii}). Conversely, at stronger orange-orange adhesion ($0.03 < \gamma_{OO}$) and weak blue-blue adhesion  ($\gamma_{BB} \approx 0$), clusters consisted of blue cells dispersed in a hexagonal configuration, surrounded by orange cells.  (\textbf{Fig.~\ref{fig:phasediagramnoprolif}b,viii}). Interestingly, this hierarchical patterning has a superficial resemblance to cone cells in the \emph{Drosophila} retina \cite{Hayashi:2004it}. At stronger orange-orange adhesion ($0.03 < \gamma_{OO}$) and slightly stronger blue-blue adhesion  ($\gamma_{BB} \approx 0.01$), clusters consisted of a core of orange cells surrounded by blue cells at the periphery (\textbf{Fig.~\ref{fig:phasediagramnoprolif}b,ix}).

At intermediate orange-blue adhesion ($\gamma_{OB} = 0.13$), with stronger blue-blue or orange-orange adhesions  ($\gamma_{OB} \le \gamma_{OO}, \gamma_{OB} \le \gamma_{BB}$), clusters again were comprised of intermixed orange and blue cells (\textbf{Fig.~\ref{fig:phasediagramnoprolif}c,v}). For weaker blue-blue or orange-orange adhesions, ($\gamma_{OO} \approx \gamma_{BB} \le \gamma_{OB}$), clusters with alternating orange and blue stripes were observed (\textbf{Fig.~\ref{fig:phasediagramnoprolif}c,vi}. At stronger blue-blue adhesion ($0.03 < \gamma_{BB}$) and weak orange-orange adhesion ($\gamma_{OO} < 0.03$), clusters consisted of orange cells dispersed in a hexagonal configuration, surrounded by tightly packed blue cells (\textbf{Fig.~\ref{fig:phasediagramnoprolif}c,xi}). Moreover, when blue-blue adhesion and orange-orange adhesion were roughly comparable ($\gamma_{BB} \approx \gamma_{OO} \approx 0.09$), clusters consisted of tightly packed orange cells dispersed in a hexagonal configuration, surrounded by tightly packed blue cells (\textbf{Fig.~\ref{fig:phasediagramnoprolif}c,x}). At the strongest blue-blue adhesion ($\gamma_{BB} \approx 0.20$) and weak orange-orange adhesion ($\gamma_{OO} < 0.03$), spots of orange cells were again dispersed in a hexagonal configuration, surrounded by slightly sparser blue cells (\textbf{Fig.~\ref{fig:phasediagramnoprolif}c,vii}). Moreover, at stronger orange-orange adhesion ($0.03 < \gamma_{OO}$) and weak blue-blue adhesion  ($\gamma_{BB} \approx 0$), clusters again consisted of blue cells dispersed in a hexagonal configuration, surrounded by orange cells.  (\textbf{Fig.~\ref{fig:phasediagramnoprolif}c,vii}). When orange-orange adhesion was comparable to orange-blue adhesion ($\gamma_{OO} \approx \gamma_{OB} =0.13$) with weaker blue-blue adhesion ($\gamma_{BB} = 0.07$), clusters were observed with finger-like or labyrinth-like patterns of orange and blue cells (\textbf{Fig.~\ref{fig:phasediagramnoprolif}c,xii}), analogous to those generated by reaction-diffusion (Turing) mechanisms \cite{Kondo:2010bx}. At strong orange-orange adhesion ($\gamma_{OO} \approx 0.2$) with weak blue-blue adhesion ($\gamma_{BB} \approx 0.03-0.11$), clusters consisted of a core of orange cells surrounded by blue cells at the periphery (\textbf{Fig.~\ref{fig:phasediagramnoprolif}c,ix}). Notably, a number of cluster configurations observed at $\gamma_{OB} = 0.13$  (\textbf{Fig.~\ref{fig:phasediagramnoprolif}c,v-ix}) were qualitatively similar to those previously observed at $\gamma_{OB} = 0.05$ (\textbf{Fig.~\ref{fig:phasediagramnoprolif}b,v-ix}), but offset to higher values of $\gamma_{BB}$ or $\gamma_{OO}$.

At strong orange-blue adhesion ($\gamma_{OB} = 0.25$) with comparable blue-blue and orange-orange adhesion ($\gamma_{BB} \approx \gamma_{OO}$), blue and orange cells organized into clusters with alternating stripes that were roughly 1-2 cells thick (\textbf{Fig.~\ref{fig:phasediagramnoprolif}d,vi}). At stronger blue-blue adhesion ($0.03 < \gamma_{BB}$) and weak orange-orange adhesion ($\gamma_{OO} < 0.03$), clusters again consisted of spots of orange cells dispersed in a hexagonal configuration, surrounded by tightly packed blue cells (\textbf{Fig.~\ref{fig:phasediagramnoprolif}c,xi}). Conversely, at stronger orange-orange adhesion ($0.03 < \gamma_{OO}$) and weak blue-blue adhesion  ($\gamma_{BB} \approx 0$), clusters again consisted of blue cells dispersed in a hexagonal configuration, surrounded by orange cells.  (\textbf{Fig.~\ref{fig:phasediagramnoprolif}d,viii}).  When orange-orange adhesion was comparable to orange-blue adhesion ($\gamma_{OO} \approx \gamma_{OB} =0.25$) with weaker blue-blue adhesion ($\gamma_{BB} = 0.15$), clusters were observed with finger-like patterns of orange and blue cells (\textbf{Fig.~\ref{fig:phasediagramnoprolif}d,xii}). Moreover, when blue-blue adhesion and orange-orange adhesion were roughly comparable ($\gamma_{BB} \approx \gamma_{OO} \approx 0.13$), clusters consisted of tightly packed orange cells dispersed in a hexagonal configuration, surrounded by tightly packed blue cells (\textbf{Fig.~\ref{fig:phasediagramnoprolif}d,x}). Finally, when all three adhesions were comparable ($\gamma_{OB} \approx \gamma_{BB} \approx \gamma_{OO} = 0.25$), clusters were observed with intermixed orange and blue cells (\textbf{Fig.~\ref{fig:phasediagramnoprolif}d,v}).

These distinct spatial patterns were classified by... \textbf{Jay fill in, comment on which approach was more successful and why}

%\textbf{William, describe observations in PHATE plots (Fig.~\ref{fig:SI_noprolif_PHATE_H1})}

\subsection{Sorting and Clustering of Two Proliferating Cell Types with Varying Adhesion}

These differential adhesion simulations were then implemented with proliferation, so that a mother would divide into two daughter after some duration (e.g. 50,000 timesteps), randomly offset. Cell division events were implemented so that one daughter retained the velocity and direction of the mother, while the other daughter was placed close to the other, but moving at equal velocity in the opposite direction. Moreover, a contact inhibition rule was included so that a cell was not permitted to divide if the local cell density was high (more than four nearest neighbors). Simulations were otherwise performed consistently with the previous scenario, starting with a 60:40 ratio of blue and orange cells while systematically varying blue-blue adhesion ($\gamma_{BB}$), orange-orange adhesion ($\gamma_{OO}$), and blue-orange adhesion  ($\gamma_{OB}$).

For weak orange-blue adhesion $\gamma_{OB} = 0.05$ with roughly comparable blue-blue and orange-orange adhesion ($\gamma_{BB} \approx \gamma_{OO}$), clusters appeared intermixed with irregular domain sizes (\textbf{Fig.~\ref{fig:phasediagramprolif}a,v}). We utilize the same numbering convention as in \textbf{Fig.~\ref{fig:phasediagramnoprolif}} for ease of comparison. Nevertheless, for weak blue-blue adhesions $\gamma_{BB} = 0.05$ and varying orange-orange adhesions $0.07 \le \gamma_{OO}$, clusters were partially sorted with more blue cells than orange cells (\textbf{Fig.~\ref{fig:phasediagramprolif}a,xiv}), which was not previously observed. By analogy,  for weak orange-orange adhesions $\gamma_{OO} = 0.05$ and varying blue-blue adhesions $0.07 \ge \gamma_{BB}$, clusters were partially sorted with more orange cells than blue cells (\textbf{Fig.~\ref{fig:phasediagramprolif}a,xv}).


\begin{figure}
    \centering
    \includegraphics[width=12cm]{figures/prolifphasediagram.png}
    \caption{\textbf{Comparison of cluster and stripe patterning for two proliferating cell types (orange, blue) with systematically varying blue-blue adhesion ($\gamma_{BB}$), orange-orange adhesion ($\gamma_{OO}$), and blue-orange adhesion  ($\gamma_{OB}$), respectively}. Representative slices with $\gamma_{BB}$ vs $\gamma_{OO}$ for $\gamma_{OB} = 0.05$ (a), $\gamma_{OB} = 0.09$ (b), $\gamma_{OB} = 0.13$ (c), $\gamma_{OB} = 0.25$ (d).}
    \label{fig:phasediagramprolif}
\end{figure}

At slightly increased orange-blue adhesion $\gamma_{OB} = 0.09$,  with roughly comparable blue-blue and orange-orange adhesion ($0.09 \le \gamma_{BB} \approx \gamma_{OO}$), clusters again appeared intermixed with irregular domain sizes (\textbf{Fig.~\ref{fig:phasediagramprolif}b,v}). In comparison, for weak blue-blue and orange-orange adhesion ($\gamma_{BB} \approx \gamma_{OO} \le 0.09 $), clusters with alternating orange and blue stripes were observed (\textbf{Fig.~\ref{fig:phasediagramprolif}b,vi}). For slightly increased blue-blue or orange-orange adhesions ($\gamma_{OO} = 0.13, \gamma_{BB} = 0.13$), clusters exhibited finger or labyrinth-like morphology (\textbf{Fig.~\ref{fig:phasediagramprolif}b,xii}). For strong blue-blue adhesions ($0.17 \le \gamma_{BB}$) and weak orange-orange adhesions ($\gamma_{OO} = 0.05$), clusters were sorted with  blue cells in the interior and orange cells at the periphery (\textbf{Fig.~\ref{fig:phasediagramprolif}b,vii}). In comparison, for strong orange-orange adhesions ($0.17 \le \gamma_{OO}$) and weak blue-blue adhesions ($\gamma_{OO} = 0.05$), clusters were sorted with  orange cells in the interior and blue cells at the periphery (\textbf{Fig.~\ref{fig:phasediagramprolif}b,ix}).

At intermediate orange-blue adhesion $\gamma_{OB} = 0.13$, with roughly comparable blue-blue and orange-orange adhesion ($0.13 \le \gamma_{BB} \approx \gamma_{OO}$), clusters continued to be intermixed with irregular domain sizes (\textbf{Fig.~\ref{fig:phasediagramprolif}c,v}). For weak orange-orange adhesions ($\gamma_{OO} < 0.13$), clusters exhibited hexagonally arrayed spots of packed orange cells surrounded by blue cells (\textbf{Fig.~\ref{fig:phasediagramprolif}c,x}). Instead, for weak blue-blue adhesions with comparable orange-orange and orange-blue adhesions ($\gamma_{BB} < \gamma_{OO} \approx \gamma_{OB} = 0.13$), clusters exhibited a stripe phase (\textbf{Fig.~\ref{fig:phasediagramprolif}c,vi}). For weak blue-blue adhesions ($\gamma_{BB} < 0.13$) with strong orange-orange adhesions ($\gamma_{OO} \approx 0.21$), clusters exhibited a labyrinth or finger-like morphology (\textbf{Fig.~\ref{fig:phasediagramprolif}c,xii}). Finally, for slightly increased blue-blue adhesion ($\gamma_{BB} = 0.09, \gamma_{OO} = 0.25$), clusters exhibited a core of orange cells with peripheral blue cells (\textbf{Fig.~\ref{fig:phasediagramprolif}c,ix}).    
At the strongest orange-blue adhesion ($\gamma_{OB} = 0.25$), intermixed clusters were only observed for comparably strong blue-blue and orange-orange adhesions ($\gamma_{BB} \approx \gamma_{OO} = 0.25$) (\textbf{Fig.~\ref{fig:phasediagramprolif}d,v}). When blue-blue and orange-orange adhesions were weaker but comparable ($\gamma_{BB} \approx \gamma_{OO} \le 0.21$), clusters with alternating orange and blue stripes were observed (\textbf{Fig.~\ref{fig:phasediagramprolif}d,vi}). At one location ($\gamma_{BB} = 0.09, \gamma_{OO} = 0.05$), clusters consisted of spots of orange cells dispersed in a hexagonal configuration, surrounded by tightly packed blue cells (\textbf{Fig.~\ref{fig:phasediagramprolif}d,xi}). For stronger blue-blue adhesions relative to orange-orange adhesions ($\gamma_{OO} < \gamma_{BB} \le 0.17$, clusters consisted of circular spots of orange cells surrounded by blue cells (\textbf{Fig.~\ref{fig:phasediagramprolif}d,x}). For weak blue-blue adhesions ($\gamma_{BB} = 0.05$), a new cluster morphology was observed with mixed stripes and spots (\textbf{Fig.~\ref{fig:phasediagramprolif}d,xii}). Finally, for stronger orange-orange adhesions relative to blue-blue adhesions ($\gamma_{BB} < \gamma_{OO} \le 0.25$, clusters exhibited a labyrinth or finger-like morphology (\textbf{Fig.~\ref{fig:phasediagramprolif}d,xii}).

These distinct spatial patterns were classified by... \textbf{Jay fill in, comment on which approach was more successful and why}
